Unsupervised Graph Anomaly Detection via Multi-Hypersphere Heterophilic Graph Learning

Graph Anomaly Detection (GAD) plays a vital role in various data mining applications such as e-commerce fraud prevention and malicious user detection. Recently, Graph Neural Network (GNN) based approach has demonstrated great effectiveness in GAD by first encoding graph data into low-dimensional representations and then identifying anomalies under the guidance of supervised or unsupervised signals. However, existing GNN-based approaches implicitly follow the homophily principle (i.e., the "like attracts like" phenomenon) and fail to learn discriminative embedding for anomalies that connect vast normal nodes. Moreover, such approaches identify anomalies in a unified global perspective but overlook diversified abnormal patterns conditioned on local graph context, leading to suboptimal performance. To overcome the aforementioned limitations, in this paper, we propose a Multi-hypersphere Heterophilic Graph Learning (MHetGL) framework for unsupervised GAD. Specifically, we first devise a Heterophilic Graph Encoding (HGE) module to learn distinguishable representations for potential anomalies by purifying and augmenting their neighborhood in a fully unsupervised manner. Then, we propose a Multi-Hypersphere Learning (MHL) module to enhance the detection capability for context-dependent anomalies by jointly incorporating critical patterns from both global and local perspectives. Extensive experiments on ten real-world datasets show that MHetGL outperforms 14 baselines. Our code is publicly available at https://github.com/KennyNH/MHetGL.

==> chapt/method_1_old.tex <==
\subsection{Heterophilic Graph Encoding}
% To address the homophily-induced indistinguishability, we aim to design a heterophilic graph encoder $\Phi_g(\cdot)$ to learn distinguishable representations for camouflaged anomalies. 

% Existing heterophilic GNNs can be categorized into two classes: (1) discriminate different neighbors, as the uniform aggregation ignores the distinction of information between similar and dissimilar neighbors; (2) extend latent neighbors, as the local aggregation fails to exploit non-local informative nodes far apart \cite{zheng2022graph}. 

% We transfer them to unsupervised GAD application and propose two strategies: (1) discriminate existing normal and abnormal neighbors for anomalies; (2) extend latent abnormal neighbors for anomalies. 

% Specifically, we propose Heterophilic Graph Encoder (HGE), which includes both a discriminating channel and an extending channel, to achieve anomaly-distinguishable representations in an unsupervised manner.

\eat{To address the homophily-induced indistinguishability, we aim to design a heterophilic graph encoder to learn distinguishable representations for anomalies linked with vast normal nodes. Existing heterophilic GNNs generally refine aggregation mechanisms with two strategies: (1) discriminate homophilic and heterophilic neighbors (i.e., with the same and different node class), as the uniform aggregation ignores the distinction of information between neighbors labeled with diverse classes; (2) discover latent homophilic neighbors, as the local aggregation fails to exploit informative nodes far apart in the graph \cite{zheng2022graph}. However, these methods require extra label information and fail to adapt to unsupervised scenarios. In this section, we introduce the proposed Heterophilic Graph Encoder (HGE) which includes two components: neighborhood refinement and anomaly-aware aggregation. To identify indistinguishable anomalies in an unsupervised manner, HGE firstly draws the inspiration from supervised heterophilic GNNs and incorporates handcrafted graph features to degrade heterophilic neighbors and discover homophilic neighbors for anomalies. Based on the refined neighborhood, anomaly-aware aggregation is executed to derive distinguishable representations for anomalies.}

\subsubsection{Homophily-guided neighborhood refinement}
\eat{Inspired by the strategies used in supervised heterophilic GNNs \cite{zheng2022graph}, we refine the neighborhood from two aspects: (1) discriminate homophilic and heterophilic neighbors, as the uniform aggregation ignores the distinction of information between neighbors labeled with diverse classes; (2) discover latent homophilic neighbors, as the local aggregation fails to exploit informative nodes far apart in the graph \cite{zheng2022graph}.}

We first elaborate how to refine the graph topology to facilitate learning distinguishable representations for graph anomalies. Concretely, our method is mainly motivated by two observations from existing literature. First, given an anomalous node, the impact of heterophilic neighbors (\ie normal neighbors) should be reduced as they introduce noisy information to the node representation~\cite{shi2022h2}. Second, anomalous nodes that exhibiting high structural and semantic similarities may sparsely distributed across the graph and distant to each other. Taking such latent relationships into account is beneficial for GAD~\cite{liu2021pick}. Motivated by these observations, we propose two training-free graph topology refinement schemes: (1) purify explicit neighbors for anomalous nodes and (2) augment latent connections between anomalous nodes. 
Notably, the ground-truth anomalous nodes are unavailable under the unsupervised GAD setting. Therefore, during the neighborhood refinement process, we choose to refine the neighbors of anomalous node candidates rather than exact anomalous nodes.
%cannot locate anomalies exactly, but select some anomalous node candidates and refine the neighbors for them.
%which are detailed as follows.

% Notably, the heterophily issue of anomalous nodes is much severer than that of normals (\eg in Reddit, the average heterophily ratio\footnote{The heterophily ratio will be introduced in Appendix~\ref{section:hetero_ratio}.} of anomalous nodes is $81.53\%$, whereas that of normal nodes is $0.55\%$). Unlike anomalous nodes, the normal nodes show strong homophily even if we do not change their neighbors. As a result, we only focus on the heterophily issue for anomalous nodes, as they are the primary cause of the homophily-induced indistinguishability.

%Notably, the ground-truth anomalous nodes are unavailable in the unsupervised GAD scenario. Therefore, during neighbor refinement, we cannot locate anomalies exactly, but select some anomalous node candidates and refine the neighbors for them.

\noindent\textbf{Explicit neighborhood purification.} 
% \eat{To discriminate heterophilic and homophilic neighbors for anomalies without supervision, we aim at attenuating the information of heterophilic neighbors and enhancing that of homophilic neighbors via adjusting the weights of existing edges. A question arising is \textsl{how to design the edge weights to discriminate heterophilic and homophilic neighbors in an unsupervised manner}? } 
Intuitively, the homophily probabilities between anomalous node and its neighbors (\ie the probabilities that the neighbors are also anomalous) are strongly correlated with the local structure characteristics. That is, the local structure around two connected anomalous nodes tend to be more complex~\cite{liu2022benchmarking}.
% To discriminate heterophilic and homophilic neighbors of anomalies in unsupervised scenarios, a plausible solution is to directly leverage traditional graph features to measure the similarities among connected nodes.
% \eat{An intuitive solution is to follow traditional GAD methods which exploit the structural property of graph anomalies for detection and require no extra label information \cite{zhao2021synergistic}.}
As validated in~\cite{chatterjee2021detecting}, graph curvature~\cite{ollivier2009ricci} can be utilized to measure the densely connected abnormal structural patterns among adjacent nodes.
Thus, we leverage graph curvature as a proxy for neighborhood purification under the unsupervised setting.
Specifically, we can calculate the graph curvature $\kappa(i,j)$ for the edge between node $v_i$ and $v_j$ by
\begin{equation}
\begin{aligned}
&\mathbf{m}_i[o]=
\begin{cases}
\tau, & v_o=v_i, \\
(1-\tau)/|\mathcal{N}|, & v_o \in \mathcal{N}, \\
0, & otherwise,\\
\end{cases}
\\ &\kappa(i,j)=1-W(\mathbf{m}_i,\mathbf{m}_j),
\end{aligned}
\label{curv}
\end{equation}
where $o=1,2,...,N$ indicates the component index of the distribution vector $\mathbf{m}$, $\tau$ is a pre-defined coefficient within $[0,1]$, $W(\cdot,\cdot)$ is the Wasserstein distance, and $\mathcal{N}$ denotes the neighbors of $v_i$ in the original graph. 
% ~\cite{villani2009wasserstein}

% The distributions of graph curvature for abnormal-abnormal and abnormal-normal edges.
\begin{figure}[t]
    \centering
    \subfloat[Edges between anomalous and normal nodes.]{\includegraphics[width=0.45\linewidth]{fig/empirical/curvs_compare_an_citeseer-syn_v1.png}}
    \hspace{5pt}
    \subfloat[Edges between anomalous nodes.]{\includegraphics[width=0.45\linewidth]{fig/empirical/curvs_compare_aa_citeseer-syn_v1.png}}
    \vspace{-5pt}
    \caption{Diverged graph curvature distribution of normal and anomalous nodes in the Citeseer dataset. The curvature of edges between anomalous nodes falls in the positive range while the majority curvature of edges between normal and anomalous nodes fall in the negative range.}
    \vspace{-12pt}
    \label{figure:motivation_1}
\end{figure}
% \includegraphics[width=0.97\linewidth]{fig/curvs_compare_citeseer-syn_v1.png}

To demonstrate the effectiveness of graph curvature based neighborhood purification, we visualize the curvature distribution of normal and anomalous nodes in the real-world Citeseer dataset~\cite{yang2016revisiting}, as depicted in Figure~\ref{figure:motivation_1}.
As can be seen, the graph curvature distributions of anomalous and normal nodes fall in significantly different ranges. Specifically, the curvature of edges between anomalous nodes tend to be positive while the curvatures among anomalous-normal edges mainly fall in a negative range\footnote{We don't report the distribution of normal-normal edges as we focus on the property of anomalies, which is interpreted in Section~\ref{section:hetero_ratio}}. Such observation supports us to utilize graph curvature as an effective proxy variable to distinguish heterophilic and homophilic neighbors of graph anomalies for neighbor purification.

%To validate our idea in a more intuitive way, we conducted an empirical study to show the properties of graph curvature, and we present our findings using the Citeseer dataset~\cite{yang2016revisiting} as an illustrative example. As depicted in Figure~\ref{figure:motivation_1}, for existing anomalous-anomalous and anomalous-normal edges, the distributions of graph curvature fall into different ranges. Specifically, the curvature values of anomalous-anomalous edges tend to be non-positive while the curvature values for anomalous-normal edges exhibit a clear opposite trend. This observation allows us to utilize graph curvature as a discriminatory metric for neighbor purification, which can distinguish between heterophilic and homophilic neighbors of graph anomalies.

Formally, given the original adjacency matrix $\mathbf{A}$, we refine the edge weights of $\mathbf{A}$ with graph curvature
\begin{equation}
\begin{aligned}
&\mathbf{A}^{pur}_{i,j}=
\begin{cases}
\kappa(i,j), & \mathbf{A}_{i,j}=1,\\
0, & \mathbf{A}_{i,j}=0,
\end{cases}\\
&\mathbf{\tilde{A}}^{pur}_{i,j}=\frac{\exp(\mathbf{A}^{pur}_{i,j})}{\sum_{j^\prime\in\tilde{\mathcal{N}}^{pur}_i}\exp(\mathbf{A}^{pur}_{i,j^\prime})},
\end{aligned}
\label{discriminate_weight}
\end{equation}
where $\tilde{\mathcal{N}}^{pur}_i=\tilde{\mathcal{N}}_i=\mathcal{N}_i\cup\{i\}$. By doing so, the edges connecting anomalies with heterophilic and homophilic neighbors are assigned with different weights, and the neighbors of anomalous nodes are purified, thus being more distinguishable. Since negative edge weights may lead to unstable model training and degrade the performance~\cite{li2022curvature}, here we apply a node-wise Softmax operation in Equation~\eqref{discriminate_weight} to normalize the weights and avoid generating the negative weights.


% The distributions of GDV similarity for abnormal-abnormal and abnormal-normal node pairs.
\begin{figure}[t]
    \centering
    \subfloat[Edges between anomalous and normal nodes.]{\includegraphics[width=0.45\linewidth]{fig/empirical/gdv_sim_an_citeseer-syn.png}}
    \hspace{5pt}
    \subfloat[Edges between anomalous nodes.]{\includegraphics[width=0.45\linewidth]{fig/empirical/gdv_sim_aa_citeseer-syn.png}}
    \vspace{-5pt}
    \caption{Diverged GDV similarity distribution of normal and anomalous nodes in the Citeseer dataset. The GDV similarity of edges between anomalous nodes follow a right-shift distribution while the GDV similarity of edges between normal and anomalous nodes follow a left-shift distribution.
    }
    \vspace{-12pt}
    \label{figure:motivation_2}
\end{figure}
% \includegraphics[width=0.97\linewidth]{fig/gdv_sim_citeseer-syn.png}

\noindent\textbf{Latent neighbor augmentation.}
% \eat{We aim to construct a new graph structure based on the latent correlation between anomalies. A question arising is \textsl{how to seek the latent correlation between anomalies to discover homophilic neighbors in an unsupervised manner}? Likewise, we focus on the structural property of graph anomalies.}
%Likewise, it is intuitive that the local structures of anomalous nodes tend to be similar.
Furthermore, to reinforce the homophilic neighbourhood aggregation effect, it can be beneficial to augment the graph structure by connecting distant anomalous nodes.
According to~\cite{harshaw2016graphprints}, a graphlet refers to a small induced subgraph that characterizes local topology, which can be leveraged to detect the occurrence of abnormal behaviors in the graph. 
%Thus we can borrow the idea of graphlet features to augment similar latent neighbors for anomalous nodes. 
In this work, we utilize the graphlet features to connect similar but distant anomalous nodes. Specifically, we count the occurrences of all surrounding graphlets consisting up to $T$ nodes for each node $v_i$, and record the values via a Graphlet Degree Vector (GDV) $\mathbf{r}_i$, to indicate the structural role of the node. For the detailed calculation of GDV, \cite{zhu2021community} could be referred to.

To illustrate the potential of GDV for anomalous node augmentation, we conduct an empirical analysis by using the Citeseer dataset~\cite{yang2016revisiting}, as reported in Figure~\ref{figure:motivation_2}. Specifically, we calculate the cosine similarity of GDVs among two arbitrary nodes, which measures the likelihood that there exists a potential connection. As can be seen, the GDV similarity of anomalous node pairs exhibits a right-shift distribution, while a left-shift distribution among anomalous-normal node pairs. In other words, anomalies tend to have higher GDV similarity with other anomalies within the graph. Thus, we choose to leverage GDV similarity to augment latent homophilic neighbors for anomalous nodes.

Formally, we first construct a binary adjacency matrix using GDV similarity based on the original adjacency matrix $\mathbf{A}$. To reduce the computational overhead, we sparsify the matrix by only preserving edges with similarity higher than a threshold $\delta$. 
In addition, it is remarkable that the similarity of GDV features are insensitive to the size of substructures (\eg the GDV similarity of two isolated nodes is $1$, while the GDV similarity of two nodes with fully-connected ego-network is also $1$). 
However, nodes with more complicated substructure should be paid more attention as they usually encompass more abnormal structural information. 
Hence, we introduce degree-based edge re-weighting to discern node pairs with varying substructure sizes and obatin the weighted structure $\mathbf{A}^{aug}$. 
Then, we normalize the weights across the neighbor set and achieve the final adjcency matrix $\mathbf{\tilde{A}}^{aug}$, which is defined as
\begin{equation}
\begin{aligned}
&\mathbf{A}^{aug}_{i,j}=
\begin{cases}
\text{sim}(\mathbf{r}_i,\mathbf{r}_j)\cdot(|\mathcal{N}_i|+|\mathcal{N}_j|), & \text{sim}(\mathbf{r}_i,\mathbf{r}_j)\geq \delta,\\
0, & otherwise,
\end{cases}\\
&\mathbf{\tilde{A}}^{aug}_{i,j}=\frac{\mathbf{A}^{aug}_{i,j}}{\sum_{j^\prime\in\tilde{\mathcal{N}}^{aug}_i}\mathbf{A}^{aug}_{i,j^\prime}},
\end{aligned}
\label{extend_weight}
\end{equation}
where $\text{sim}(\cdot,\cdot)$ is cosine similarity function and $\delta$ denotes the threshold for sparsification. $\tilde{\mathcal{N}}^{aug}_i=\mathcal{N}^{aug}_i\cup\{i\}$ and $\mathcal{N}^{aug}_i$ denotes the neighbor set of node $v_i$ in the augmented graph constructed by GDV similarity.

% We can formulate $\mathbf{A}^{aug}$ as
% \begin{equation}
% \mathbf{A}^{aug}_{i,j}=
% \begin{cases}
% 1, & \text{sim}(\mathbf{r}_i,\mathbf{r}_j)\geq \delta,\\
% 0, & otherwise,
% \end{cases}
% \label{gdv_mat}
% \end{equation}

% Specifically, we normalize the weights across the neighbor set and transform the matrix $\mathbf{A}^{aug}$ into the weighted form $\mathbf{A}^{aug}$, which is defined as
% \begin{equation}
% \begin{aligned}
% &\mathbf{A}^{aug}_{i,j}=
% \begin{cases}
% |\mathcal{N}^{aug}_i|+|\mathcal{N}^{aug}_j|, & \mathbf{A}^{aug}_{i,j}=1,\\
% 0, & \mathbf{A}^{aug}_{i,j}=0,
% \end{cases}\\
% &\mathbf{\tilde{A}}^{aug}_{i,j}=\frac{\mathbf{A}^{aug}_{i,j}}{\sum_{j^\prime\in\tilde{\mathcal{N}}^{aug}_i}\mathbf{A}^{aug}_{i,j^\prime}}.
% \end{aligned}
% \label{extend_weight}
% \end{equation}

\subsubsection{Anomaly-aware aggregation}
\eat{Based on the refined neighborhood represented by weighted graph structure $\mathbf{A}^{pur}$ and $\mathbf{A}^{aug}$, anomaly-aware aggregation is introduced for generating distinguishable representations. Specifically, we respectively apply anomaly-aware aggregation in $\mathbf{A}^{pur}$ and $\mathbf{A}^{aug}$, then fuse the two hidden outputs into the final representations.}
Building upon the refined graph structure, we propose an anomaly-aware aggregation module to generate distinguishable node embeddings. Specifically, we first employ $\mathbf{\tilde{A}}^{pur}$ and $\mathbf{\tilde{A}}^{aug}$ for anomaly-aware aggregation, then fuse the outputs to produce the final representations.

Here we take $\mathbf{\tilde{A}}^{pur}$ for illustration, the process on $\mathbf{\tilde{A}}^{aug}$ is similar. 
Specifically, we propose a two-fold aggregation operator to obtain representations~\cite{wijesinghe2021new} to exploit the anomaly-aware structural information and adaptively learn implicit neighbor correlation simultaneously. Concretely, the inputs of our aggregation module include the weighted adjacency matrix $\mathbf{\tilde{A}}^{pur}$ and the hidden representations $\mathbf{\tilde{h}}_i^{(l-1)}\in\mathbb{R}^d$ of node $v_i$ at layer $l-1$, where $d$ denotes the hidden dimension and $\mathbf{\tilde{h}}_i^{(0)}=\mathbf{x}_i\in\mathbb{R}^{d_{in}}$. To distinguish the anomalous nodes from normal ones, we aggregate the hidden representations with the anomaly-aware weights in the refined neighborhood
\begin{equation}
\begin{aligned}
{\mathbf{h}_i^{pur}}^{(l)}=\gamma^{(l)}\cdot \mathbf{\tilde{h}}_i^{(l-1)}+\sum_{j\in \mathcal{N}^{pur}_i} \frac{1+\mathbf{\tilde{A}}^{pur}_{i,j}}{\sqrt{|\tilde{\mathcal{N}}^{pur}_i||\tilde{\mathcal{N}}^{pur}_j|}}\cdot \mathbf{\tilde{h}}_j^{(l-1)},
\end{aligned}
\label{aggregation}
\end{equation}
where the coefficient $\mathbf{\gamma}^{(l)}\in\mathbb{R}$ is trainable. Then we further employ an attention layer to quantify the importance of different neighbors for aggregation, which is defined as
\begin{equation}
\begin{aligned}
&{\mathbf{\tilde{h}}_i^{pur}}^{(l)}=\sum_{j\in \tilde{\mathcal{N}}^{pur}_i}\alpha_{i,j}\cdot\mathbf{W}^{(l)}{\mathbf{h}_j^{pur}}^{(l)},\\
&\alpha_{i,j}=\frac{\exp(\text{ReLU}(\mathbf{a}^{(l)}\cdot[\mathbf{W}^{(l)}{\mathbf{h}_i^{pur}}^{(l)}||\mathbf{W}^{(l)}{\mathbf{h}_j^{pur}}^{(l)}]))}{\sum_{j^\prime\in \tilde{\mathcal{N}}^{pur}_i}\exp(\text{ReLU}(\mathbf{a}^{(l)}\cdot[\mathbf{W}^{(l)}{\mathbf{h}_i^{pur}}^{(l)}||\mathbf{W}^{(l)}{\mathbf{h}_{j^\prime}^{pur}}^{(l)}]))},
\end{aligned}
\label{gat}
\end{equation}
where $\mathbf{W}^{(l)},\mathbf{a}^{(l)}$ are trainable parameters and ${\mathbf{\tilde{h}}_i^{pur}}^{(l)}\in\mathbb{R}^d$ denotes the hidden representation of node $v_i$ in the $l$-th layer.
Similarly, based on $\mathbf{A}^{aug}$ and the hidden representations $\mathbf{\tilde{h}}_i^{(l-1)}$. We apply the anomaly-aware aggregation and obtain the output ${\mathbf{\tilde{h}}_i^{aug}}^{(l)}$.

Subsequently, we combine the node representations to derive the final representation to enhance the expressivity
\begin{equation}
\mathbf{\tilde{h}}_i^{(l)}=\mathbf{W}^{(l)}[{\mathbf{\tilde{h}}_i^{pur}}^{(l)}||\ {\mathbf{\tilde{h}}_i^{aug}}^{(l)}]+\mathbf{b}^{(l)},
\label{mlp}
\end{equation}
where $\mathbf{W}^{(l)},\mathbf{b}^{(l)}$ are trainable parameters. We define the output of the last layer as $\mathbf{z}_i=\mathbf{\tilde{h}}_i^{(L)}\in\mathbb{R}^d$, which will be utilized in the MHL module introduced below.

% \subsubsection{Discriminating channel} 
% The discriminating channel includes two components: (1) anomaly-wise neighbor discrimination; (2) structure-aware aggregation.

% \noindent\textbf{Anomaly-wise neighbor discrimination.} To discriminate different neighbors for anomalies without supervision, we aim at assigning distinct structural coefficients for them. A question arising is \textsl{how to design anomaly-aware coefficients to discriminate distinct neighbors in a parameter-free way}? 

% An intuitive solution is to focus on the structural property of anomalies in the graph which requires no extra trainable parameters. Inspired by \cite{chatterjee2021detecting}, graph curvature can be used to identify abnormal structural patterns, which measures how easily information flows between two nodes \cite{ye2019curvature,li2022curvature} compared to traditional features (e.g. clustering coefficients). Following \cite{ollivier2009ricci,coupette2022ollivier}, graph curvature $\kappa(i,j)$ for each edge between node $v_i$ and $v_j$ is computed as follows:
% \begin{equation}
% \begin{aligned}
% &\mathbf{m}_i[o]=
% \begin{cases}
% \tau, & v_o=v_i, \\
% (1-\tau)/|\mathcal{N}^{pur}_i|, & v_o \in \mathcal{N}^{pur}_i, \\
% 0, & otherwise,\\
% \end{cases}
% \\ &\kappa(i,j)=1-W(m_i,m_j),
% \end{aligned}
% \label{curv}
% \end{equation}
% where $o=1,2,...,N$, $\tau$ is a weight parameter within $[0,1]$, and $W(\cdot,\cdot)$ is Wasserstein distance measure. $\mathcal{N}^{pur}_i$ denotes the neighbors of $v_i$. To study the potentials for solving the indistinguishability, we explore the properties of graph curvature with an empirical study in Citeseer dataset \cite{yang2016revisiting}. As illustrated in Figure~\ref{figure:motivation_1}, for existing abnormal-abnormal and abnormal-normal edges, the distributions of the edge-based curvature fall into distinct ranges. Specifically, the curvature values of abnormal-abnormal edges tend to be non-positive while the curvature values of abnormal-normal edges are just the opposite. Therefore, we could intuitively use graph curvature to discriminate existing normal and abnormal neighbors for anomalies. Notably, in this work, we only focus on the heterophily issue for abnormal nodes, as they are the primary contributors to the homophily-induced indistinguishability. Specifically, the heterophily issue of abnormal nodes is much severer than that of normals (e.g., in Reddit, the average heterophily ratio\footnote{The heterophily ratio will be introduced in Appendix \ref{section:hetero_ratio}.} of abnormal nodes is $81.53\%$, whereas that of normals is $0.55\%$). Unlike abnormal nodes, most neighbors of normal nodes are also normal, demonstrating good distinguishability.

% Specifically, we define the binary adjacency matrix as $\mathbf{A}^{pur}=\mathbf{A}$ where the subscript $I$ characterizes the discriminating channel. Then we can design the structural coefficients (i.e., edge weights) with graph curvature as follows:
% \begin{equation}
% \begin{aligned}
% &\mathbf{A}^{pur}_{i,j}=
% \begin{cases}
% \kappa(i,j), & \mathbf{A}^{pur}_{i,j}=1,\\
% 0, & \mathbf{A}^{pur}_{i,j}=0,
% \end{cases}\\
% &\mathbf{\tilde{A}}^{pur}_{i,j}=\frac{\exp(\mathbf{A}^{pur}_{i,j})}{\sum_{j^\prime\in\tilde{\mathcal{N}}^{pur}_i}\exp(\mathbf{A}^{pur}_{i,j^\prime})},
% \end{aligned}
% \label{discriminate_weight}
% \end{equation}
% where $\tilde{\mathcal{N}}^{pur}_i=\mathcal{N}^{pur}_i\cup\{i\}$ and we obtain $\mathbf{\tilde{A}}^{pur}$ which is the weighted form of $\mathbf{A}^{pur}$. Here we apply a node-wise Softmax operation to normalize the weights and avoid the negative edge weights which are proved to exacerbate the difficulty of model training and degrade the performance~\cite{li2022curvature}.

% \noindent\textbf{Structure-aware aggregation.} Inspired by \cite{wijesinghe2021new}, we propose a two-fold aggregation formula to fully exploit the rich anomaly-aware structural coefficients. Specifically, we will input the weighted adjacency matrix $\mathbf{\tilde{A}}^{pur}$ and the hidden representations $\mathbf{\tilde{h}}_i^{(l-1)}\in\mathbb{R}^d,\ i=1,2,...,|\mathcal{V}|$ obtained from the last layer where the current layer $l\in\{1,2,...,L\}$, $L$ is the number of layers and $d$ denotes the hidden dimension. For the first layer, $\mathbf{\tilde{h}}_i^{(0)}=\mathbf{x}_i\in\mathbb{R}^{d_{in}}$. Firstly, we aggregate the hidden representations with the anomaly-aware weights as follows:
% \begin{equation}
% \begin{aligned}
% {\mathbf{h}_i^{pur}}^{(l)}=\mathbf{\gamma}^{(l)}\cdot \mathbf{\tilde{h}}_i^{(l-1)}+\sum_{j\in \mathcal{N}^{pur}_i} \frac{1+\mathbf{\tilde{A}}^{pur}_{i,j}}{\sqrt{|\tilde{\mathcal{N}}^{pur}_i||\tilde{\mathcal{N}}^{pur}_j|}}\cdot \mathbf{\tilde{h}}_j^{(l-1)},
% \end{aligned}
% \label{aggregation}
% \end{equation}
% where the coefficient $\mathbf{\gamma}^{(l)}\in\mathbb{R}$ is trainable. Then we employ an attention layer formulated as follows:
% \begin{equation}
% \begin{aligned}
% &{\mathbf{\tilde{h}}_i^{pur}}^{(l)}=\sum_{j\in \tilde{\mathcal{N}}^{pur}_i}\alpha_{i,j}\cdot\mathbf{W}^{(l)}{\mathbf{h}_j^{pur}}^{(l)},\\
% &\alpha_{i,j}=\frac{\exp(\text{ReLU}(\mathbf{a}^{(l)}\cdot[\mathbf{W}^{(l)}{\mathbf{h}_i^{pur}}^{(l)}||\mathbf{W}^{(l)}{\mathbf{h}_j^{pur}}^{(l)}]))}{\sum_{j^\prime\in \tilde{\mathcal{N}}^{pur}_i}\exp(\text{ReLU}(\mathbf{a}^{(l)}\cdot[\mathbf{W}^{(l)}{\mathbf{h}_i^{pur}}^{(l)}||\mathbf{W}^{(l)}{\mathbf{h}_{j^\prime}^{pur}}^{(l)}]))},
% \end{aligned}
% \label{gat}
% \end{equation}
% where $\mathbf{W}^{(l)},\mathbf{a}^{(l)}$ are trainable parameters and ${\mathbf{\tilde{h}}_i^{pur}}^{(l)}\in\mathbb{R}^d$ denotes the hidden representation of node $v_i$ of the discriminating channel in the $l$-th layer.

% \subsubsection{Extending channel} 
% The extending channel includes two components: (1) anomaly-wise neighbor extension; (2) structure-aware aggregation.

% \noindent\textbf{Anomaly-wise neighbor extension.} To extend latent neighbors for anomalies in an unsupervised manner, we aim to construct a new graph structure with more edges between anomalies. A question arising is \textsl{how to find latent correlation between anomalies to extend neighbors in a parameter-free way}? 

% Likewise, we focus on the structural property of graph anomalies. Inspired by \cite{harshaw2016graphprints}, graphlet counts will be affected by the occurrence of abnormal behaviors in the network, where graphlet is defined by small, connected and induced subgraph that describe local topology. For each node $v_i$, we count occurrences of all surrounding graphlets up to size $5$, and store the counts in a
% graphlet degree vector (GDV), denoted $\mathbf{r}_i$,  which indicates the structural role of the node \cite{zhu2021community}. To study the potentials for solving the indistinguishability, we explore the properties of GDV with an empirical study in Citeseer dataset \cite{yang2016revisiting}. Specifically, to seek latent correlation between nodes, we use cosine similarity to calculate the pairwise similarity of GDVs $\mathbf{r}_i,i=1,2,...,N$, which indicates the probability that there exists the potential connection between each node pair. As is illustrated in Figure~\ref{figure:motivation_2}, the distribution of the GDV similarity of abnormal-abnormal node pairs presents a right-shift characteristic, compared to that of abnormal-normal node pairs. In other words, anomalies will present higher GDV similarity with anomalies in the graph compared to normals. Thus intuitively we could use GDV similarity to extend latent abnormal neighbors for anomalies. 

% Specifically, we build a new binary adjacency matrix $\mathbf{A}^{aug}$ with GDV similarity based on the raw binary structure $\mathbf{A}$, where the subscript $II$ characterizes the extending channel. Since fully-connected adjacency matrix usually makes little sense for representation learning and also brings about expensive computation cost \cite{liu2022towards}, we conduct sparsification and only retain node pairs with high similarity values and construct an edge between nodes in each pair. We can formulate $\mathbf{A}^{aug}$ as follows:
% \begin{equation}
% \mathbf{A}^{aug}_{i,j}=
% \begin{cases}
% 1, & \text{Sim}(\mathbf{r}_i,\mathbf{r}_j)=1,\\
% 0, & otherwise,
% \end{cases}
% \label{gdv_mat}
% \end{equation}
% where $\text{Sim}(\cdot,\cdot)$ is cosine similarity function. Notably, the similarity of GDV features are insensitive to the size of substructures. For instance, the GDV similarity of two isolated nodes is $1$, while the GDV similarity of two nodes with fully-connected ego-network is also $1$. However, nodes with more complicated substructure should be paid more attention as they usually embody richer structural information. Therefore, we construct degree-based edge weights to differentiate node pairs with distinct sizes of substructures. The matrix $\mathbf{A}^{aug}$ can be extended to the following weighted form:
% \begin{equation}
% \begin{aligned}
% &\mathbf{A}^{aug}_{i,j}=
% \begin{cases}
% |\mathcal{N}^{aug}_i|+|\mathcal{N}^{aug}_j|, & \mathbf{A}^{aug}_{i,j}=1,\\
% 0, & \mathbf{A}^{aug}_{i,j}=0,
% \end{cases}\\
% &\mathbf{\tilde{A}}^{aug}_{i,j}=\frac{\mathbf{A}^{aug}_{i,j}}{\sum_{j^\prime\in\tilde{\mathcal{N}}^{aug}_i}\mathbf{A}^{aug}_{i,j^\prime}},
% \end{aligned}
% \label{extend_weight}
% \end{equation}
% where we normalize the weights across the neighbor set.

% \noindent\textbf{Structure-aware aggregation.} Similar to the discriminating channel, we input $\mathbf{A}^{aug}$ and the hidden representations $\mathbf{\tilde{h}}_i^{(l-1)}$. We apply the structure-aware aggregation in Equation~\ref{aggregation} and \ref{gat} and obtain the hidden representations ${\mathbf{\tilde{h}}_i^{aug}}^{(l)}$ in the extending channel.

% \subsubsection{Corssed-channel fusion} 
% To jointly capture the information in discriminating and extending channels, we fuse the node representations in a crossed way. Specifically, we use a linear network to wheld the representations of two channels together as follows:
% \begin{equation}
% \mathbf{\tilde{h}}_i^{(l)}=\mathbf{W}^{(l)}[{\mathbf{\tilde{h}}_i^{pur}}^{(l)}||\ {\mathbf{\tilde{h}}_i^{aug}}^{(l)}]+\mathbf{b}^{(l)},
% \label{mlp}
% \end{equation}
% where $\mathbf{W}^{(l)},\mathbf{b}^{(l)}$ are trainable. We define the output of the last layer as $\mathbf{z}=\mathbf{\tilde{h}}^{(L)}\in\mathbb{R}^d$.

% % \subsubsection{Method motivation} \label{section:motivation}
% % Note that the heterophily issue of abnormal nodes is much severer than that of normals (e.g., in Reddit, the average heterophily ratio\footnote{The heterophily ratio will be introduced in Appendix \ref{section:hetero_ratio}.} of abnormal nodes is $81.53\%$, whereas that of normals is $0.55\%$). Unlike abnormal nodes, most neighbors of normal nodes are also normal, demonstrating good distinguishability. So in this work, we only focus on the heterophily issue for abnormal nodes, as they are the primary contributors to the homophily-induced indistinguishability. To address this issue, we follow existing two general strategies in heterophily-against GNNS \cite{zheng2022graph} and apply them to the anomaly detection application: (1) discriminate existing normal and abnormal neighbors for anomalies; (2) extend latent abnormal neighbors for anomalies.

% % Then we show the motivations of how to achieve the two goals above. Traditional GAD methods usually use handcrafted features for anomaly detection \cite{ma2021comprehensive}. Inspired by existing works \cite{chatterjee2021detecting,harshaw2016graphprints}, we explore the properties of two structural features: graph curvature \cite{ollivier2009ricci} and graph degree curvature (GDV) \cite{prvzulj2004modeling}, for their effectiveness in GAD. We take Citeseer dataset \cite{yang2016revisiting} as an example and the empirical study below shows potentials to tackle the homophily-induced indistinguishability with these features.

% % \noindent\textbf{Motivation 1.} Compared to traditional features (e.g. clustering coefficients), graph curvature measures how easily information flows between two nodes \cite{ye2019curvature,li2022curvature}, which can be used to identify abnormal structural patterns \cite{chatterjee2021detecting}. For each link in the graph, we can calculate an edge-based curvature value (which will be introduced below). As illustrated in Figure~\ref{figure:motivation_1}, for existing abnormal-abnormal and abnormal-normal edges, the distributions of the edge-based curvature fall into distinct ranges. Specifically, the curvature values of abnormal-abnormal edges tend to be non-positive while the curvature values of abnormal-normal edges are just the opposite. Therefore, we could intuitively use graph curvature to discriminate existing normal and abnormal neighbors for anomalies.

% % \noindent\textbf{Motivation 2.} Graphlet degree curvature (GDV) is a graphlet-based node feature indicating the structural role of the node \cite{zhu2021community}, which can be used to detect structural anomalies in the graph \cite{harshaw2016graphprints}. We can calculate the GDV (which will be introduced below) for each node and the pair-wise GDV similarity is computed with the GDVs of any two nodes in the graph. As is illustrated in Figure~\ref{figure:motivation_2}, the distribution of the GDV similarity of abnormal-abnormal node pairs presents a right-shift characteristic, compared to that of abnormal-normal node pairs. In other words, anomalies will present higher GDV similarity with anomalies in the graph compared to normals. Thus intuitively we could use GDV similarity to extend latent abnormal neighbors for anomalies. 

% % \noindent\textbf{Structure construction.} For the graph structure in the discriminating channel, we directly use the raw adjacency matrix $\mathbf{A}^{pur}=\mathbf{A}$ where the subscript $I$ characterizes the discriminating channel.

% % \noindent\textbf{Weight construction.} Based on the motivation described in Section \ref{section:motivation}, we utilize graph curvature as the edge weight, to discriminate existing normal and abnormal neighbors for anomalies. Following \cite{ollivier2009ricci,coupette2022ollivier}, we compute the graph curvature $\kappa(i,j)$ for each edge between node $v_i$ and $v_j$ as follows:
% % \begin{equation}
% % \begin{aligned}
% % &\mathbf{m}_i[o]=
% % \begin{cases}
% % \tau, & v_o=v_i, \\
% % (1-\tau)/|\mathcal{N}^{pur}_i|, & v_o \in \mathcal{N}^{pur}_i, \\
% % 0, & otherwise,\\
% % \end{cases}
% % \\ &\kappa(i,j)=1-W(m_i,m_j),
% % \end{aligned}
% % \label{curv}
% % \end{equation}
% % where $o=1,2,...,N$, $W(\cdot,\cdot)$ is Wasserstein distance measure and $\tau$ is a weight parameter within $[0,1]$. $\mathcal{N}^{pur}_i$ denotes the neighbors of $v_i$. Then we can transform the raw adjacency matrix $\mathbf{A}^{pur}$ to a weighted form $\mathbf{\tilde{A}}^{pur}$ as follows:
% % \begin{equation}
% % \begin{aligned}
% % &\mathbf{A}^{pur}_{i,j}=
% % \begin{cases}
% % \kappa(i,j), & \mathbf{A}^{pur}_{i,j}=1,\\
% % 0, & \mathbf{A}^{pur}_{i,j}=0,
% % \end{cases}\\
% % &\mathbf{\tilde{A}}^{pur}_{i,j}=\frac{\exp(\mathbf{A}^{pur}_{i,j})}{\sum_{j^\prime\in\tilde{\mathcal{N}}^{pur}_i}\exp(\mathbf{A}^{pur}_{i,j^\prime})},
% % \end{aligned}
% % \label{discriminate_weight}
% % \end{equation}
% % where $\tilde{\mathcal{N}}^{pur}_i=\mathcal{N}^{pur}_i\cup\{i\}$. Here we apply a node-wise Softmax operation to normalize the weights and avoid the negative edge weights which are proved to exacerbate the difficulty of model training and degrade the performance~\cite{li2022curvature}. 

% % % Note that our proposed method is GNN-agnostic. specifically, we can use any message passing-based GNN as the backbone. In this work, we use GAT \cite{gat} as an instance.
% % \noindent\textbf{Graph convolution.} Inspired by \cite{wijesinghe2021new}, we propose an anomaly structure-aware graph convolutional network, \textsl{AnoStrGCN}, with a two-fold architecture to fully exploit the rich structural weights. Specifically, we will input the weighted adjacency matrix $\mathbf{\tilde{A}}^{pur}$ and the hidden representations $\mathbf{\tilde{h}}_i^{(l-1)}\in\mathbb{R}^d,\ i=1,2,...,|\mathcal{V}|$ obtained from the last layer where the current layer $l\in\{1,2,...,L\}$, $L$ is the number of layers and $d$ denotes the hidden dimension. For the first layer, $\mathbf{\tilde{h}}_i^{(0)}=\mathbf{x}_i\in\mathbb{R}^{d_{in}}$. Firstly, we aggregate the hidden representations based on constructed edge weights as follows:
% % \begin{equation}
% % \begin{aligned}
% % {\mathbf{h}_i^{pur}}^{(l)}=\mathbf{\gamma}^{(l)}\cdot \mathbf{\tilde{h}}_i^{(l-1)}+\sum_{j\in \mathcal{N}^{pur}_i} \frac{1+\mathbf{\tilde{A}}^{pur}_{i,j}}{\sqrt{|\tilde{\mathcal{N}}^{pur}_i||\tilde{\mathcal{N}}^{pur}_j|}}\cdot \mathbf{\tilde{h}}_j^{(l-1)},
% % \end{aligned}
% % \label{aggregation}
% % \end{equation}
% % where the coefficient $\mathbf{\gamma}^{(l)}\in\mathbb{R}$ is trainable. Then we employ an attention layer formulated as follows:
% % \begin{equation}
% % \begin{aligned}
% % &{\mathbf{\tilde{h}}_i^{pur}}^{(l)}=\sum_{j\in \tilde{\mathcal{N}}^{pur}_i}\alpha_{i,j}\cdot\mathbf{W}^{(l)}{\mathbf{h}_j^{pur}}^{(l)},\\
% % &\alpha_{i,j}=\frac{\exp(\text{ReLU}(\mathbf{a}^{(l)}\cdot[\mathbf{W}^{(l)}{\mathbf{h}_i^{pur}}^{(l)}||\mathbf{W}^{(l)}{\mathbf{h}_j^{pur}}^{(l)}]))}{\sum_{j^\prime\in \tilde{\mathcal{N}}^{pur}_i}\exp(\text{ReLU}(\mathbf{a}^{(l)}\cdot[\mathbf{W}^{(l)}{\mathbf{h}_i^{pur}}^{(l)}||\mathbf{W}^{(l)}{\mathbf{h}_{j^\prime}^{pur}}^{(l)}]))},
% % \end{aligned}
% % \label{gat}
% % \end{equation}
% % where $\mathbf{W}^{(l)},\mathbf{a}^{(l)}$ are trainable parameters and ${\mathbf{\tilde{h}}_i^{pur}}^{(l)}\in\mathbb{R}^d$ denotes the hidden representation of node $v_i$ of the discriminating channel.

% % \subsubsection{Extending channel} Likewise, the extending channel includes three steps and we implement the first two steps in advance.

% % \noindent\textbf{Structure construction.} For the graph structure in the extending channel, we build a new adjacency matrix $\mathbf{A}^{aug}$ based on the raw structure $\mathbf{A}$, where the subscript $II$ characterizes the extending channel. Based on the motivation described in Section \ref{section:motivation}, we utilize GDV similarity to discover latent abnormal neighbors for anomalies. Specifically, for each node $v_i$, we compute the GDV feature $\mathbf{r}_i$ and then use cosine similarity to calculate the pairwise similarity of features $\mathbf{r}_i,i=1,2,...,N$, which indicates the probability that there exists the potential connection between each node pair. Since fully-connected adjacency matrix usually makes little sense for representation learning and also brings about expensive computation cost \cite{liu2022towards}, we conduct sparsification and only retain node pairs with high similarity values and construct an edge between nodes in each pair. We can formulate $\mathbf{A}^{aug}$ as follows:
% % \begin{equation}
% % \mathbf{A}^{aug}_{i,j}=
% % \begin{cases}
% % 1, & \text{Sim}(\mathbf{r}_i,\mathbf{r}_j)=1,\\
% % 0, & otherwise,
% % \end{cases}
% % \label{gdv_mat}
% % \end{equation}
% % where $\text{Sim}(\cdot,\cdot)$ is cosine similarity function.

% % \noindent\textbf{Weight construction.} The similarity of GDV features are insensitive to the size of substructures. For instance, the GDV similarity of two isolated nodes is $1$, while the GDV similarity of two nodes with fully-connected ego-network is also $1$. However, nodes with more complicated substructure should be paid more attention as they usually embody richer structural information. Therefore, we construct degree-based edge weights to differentiate node pairs with distinct sizes of substructures. The matrix $\mathbf{A}^{aug}$ can be extended to the following weighted form:
% % \begin{equation}
% % \begin{aligned}
% % &\mathbf{A}^{aug}_{i,j}=
% % \begin{cases}
% % |\mathcal{N}^{aug}_i|+|\mathcal{N}^{aug}_j|, & \mathbf{A}^{aug}_{i,j}=1,\\
% % 0, & \mathbf{A}^{aug}_{i,j}=0,
% % \end{cases}\\
% % &\mathbf{\tilde{A}}^{aug}_{i,j}=\frac{\mathbf{A}^{aug}_{i,j}}{\sum_{j^\prime\in\tilde{\mathcal{N}}^{aug}_i}\mathbf{A}^{aug}_{i,j^\prime}},
% % \end{aligned}
% % \label{extend_weight}
% % \end{equation}
% % where we normalize the weights across the neighbor set.

% % \noindent\textbf{Graph convolution.} Similar to the discriminating channel, we input the hidden representations $\mathbf{\tilde{h}}_i^{(l-1)}$ from the last layer. We apply the same graph convolution in Equation~\ref{aggregation} and \ref{gat} and obtain the hidden representations ${\mathbf{\tilde{h}}_i^{aug}}^{(l)}$ in the extending channel.

% % To jointly capture the information in discriminating and extending channels, we fuse the node representations in a crossed way. Specifically, we use a linear network to wheld the representations of two channels together as follows:
% % \begin{equation}
% % \mathbf{\tilde{h}}_i^{(l)}=\mathbf{W}^{(l)}[{\mathbf{\tilde{h}}_i^{pur}}^{(l)}||\ {\mathbf{\tilde{h}}_i^{aug}}^{(l)}]+\mathbf{b}^{(l)},
% % \label{mlp}
% % \end{equation}
% % where $\mathbf{W}^{(l)},\mathbf{b}^{(l)}$ are trainable. We define the output of the last layer as $\mathbf{z}=\mathbf{\tilde{h}}^{(L)}\in\mathbb{R}^d$.




